The optimality of (stochastic) veto delegation

We analyze the optimal delegation problem between a principal and an agent, assuming that the latter has state-independent preferences. We demonstrate that if the principal is more risk-averse than the agent toward non-status quo options, an optimal mechanism is a {\em veto mechanism}. In a veto mechanism, the principal uses veto (i.e., maintaining the status quo) to balance the agent's incentives and does not randomize among non-status quo options. We characterize the optimal veto mechanism in a one-dimensional setting. In the solution, the principal uses veto only when the state surpasses a critical threshold.

==> legislative.tex <==
\section{Application to legislative rules}
\label{sec-application}

Our model can be applied to gain new insights in the design of the legislative rules.
Most previous works on legislative rules, such as
Gilligan and Krehbiel (1987,1989) and Krishna and Morgan~(2001),
take the rules as given and study the informational efficiency of the \textit{closed rule} and the \textit{open rule}.  
Alonso and Matouschek~(2008) adopt the mechanism design approach, but their identified optimal legislative rule takes the interval delegation
form, which is different from both the closed rule and the open rule.
Our framework supports the superiority of the closed rule, given that the principal can pre-commit to the veto probabilities conditional on the agent's proposals.

\paragraph{Model}
The committee (Agent) makes a proposal to the legislature (Principal) 
regarding which policy to adopt.
The legislature's utility is determined by both the state $\state \in [0,1]$ and the enacted policy $a \in (-\infty, 2] \cup \set{\an}$, where $\an$ means maintaining the status quo.
The committee's utility function $v(a)$ and the legislature's utility functions $u(a,\state)$ are given by:
\[
\begin{split}
	v(a) = \begin{cases}
		a & \text{if } a \in (-\infty, 2]; \\
		0 & \text{if } a = \an, 
	\end{cases}
\qquad %
   	u(a, \theta) = \begin{cases}
		-(a - \theta)^2 & \text{if } a \in (-\infty, 2]; \\
		-0.2 & \text{if } a = \an. 
	\end{cases}
\end{split}
\]
Note that the committee is extremely biased and prefers higher policies regardless of the state.

The committee privately observes the state $\theta$. 
The legislature does not know the state and his prior belief is that $\theta$ is uniformly distributed.
The legislature can commit to any (stochastic) decision rule.
These rules include
(i) the {open rule} under which the legislature 
%chooses some active policy other than the one proposed by the committee with positive probability;
is free to enact any new policy or maintain the status quo and
(ii) the {closed rule} under which the legislature either accepts a proposal or rejects for the status quo policy.

\paragraph{Optimal legislative rule}

%\Cref{prp-main-result}, 
%\begin{equation}
%\begin{aligned}
%        \amap^*(\theta)  
%          \begin{cases}
%          \approx {0.394},  & \text{ if } \theta < 0.596 \\
%          = \sqrt{\theta^2 -0.2} , & \text{ if } \theta \ge 0.596
%          \end{cases}
% \qquad\qquad %
%      \pmap^*(\theta) 
%        \begin{cases}
%           = 0,  & \text{ if } \theta < 0.596 \\
%          \approx \frac{\sqrt{\theta^2 -0.2} -  0.394}{\sqrt{\theta^2 -0.2}} , & \text{ if } \theta \ge 0.596 
%        \end{cases}
%    \label{eq:optim-veto} 
%\end{aligned}
%\end{equation}

Previous analysis indicates that it is without loss to focus on 
veto mechanisms, and the optimal veto mechanism is achieved 
by the veto delegation arrangement.
In particular, an optimal legislative rule is as follows:
the legislature commits to always approving any proposal from $[0,0.394]$;\footnotemark{}
approving the proposal $a \in ( 0.394 , \sqrt{0.8}]$ with probability $\frac{0.394}{a}$ and using veto with the complementary probability;
otherwise always using veto.
As a result, this optimal legislative rule corresponds to the {closed rule}.

\footnotetext{%
  Here $0.394$ is an approximate solution to 
  $\int_{\sqrt{a^2 +0.2}}^1 (\sqrt{\theta^2 - 0.2} - a) \, d \theta +a - \frac{1}{2} = 0.$
}

